Deep Just-In-Time Inconsistency Detection Between Comments and Source Code

Natural language comments convey key aspects of source code such as implementation, usage, and pre- and post-conditions. Failure to update comments accordingly when the corresponding code is modified introduces inconsistencies, which is known to lead to confusion and software bugs. In this paper, we aim to detect whether a comment becomes inconsistent as a result of changes to the corresponding body of code, in order to catch potential inconsistencies just-in-time, i.e., before they are committed to a code base. To achieve this, we develop a deep-learning approach that learns to correlate a comment with code changes. By evaluating on a large corpus of comment/code pairs spanning various comment types, we show that our model outperforms multiple baselines by significant margins. For extrinsic evaluation, we show the usefulness of our approach by combining it with a comment update model to build a more comprehensive automatic comment maintenance system which can both detect and resolve inconsistent comments based on code changes.

==> Makefile <==
formattedS := formatted
TEXS := $(wildcard *.tex)
TABLES := $(wildcard tables/**/*.tex)
FIGS := $(wildcard figs/*.tex) $(wildcard images/*.png) $(wildcard images/*.PNG) $(wildcard code/*)
PLOTS := $(wildcard figs/*.eps)
BIBS := $(wildcard *.bib)

LATEX = pdflatex -interaction=nonstopmode
BIBTEX = bibtex

.PHONY: all
all: $(formattedS:=.pdf)

.PHONY: display
display: $(formattedS:=.pdf)
	evince $(formattedS:=.pdf)

$(formattedS:=.pdf) : %.pdf : ${TEXS} ${TABLES} ${BIBS} ${FIGS} ${PLOTS}
	-rm -f $*.aux
	-rm -f $*.bbl
	-$(LATEX) $*
	-$(BIBTEX) $*
	-$(LATEX) $*
	-$(LATEX) $*
# Check error
	@if [ -z "$$(grep -i "error" formatted.log | grep -v "errmessage" | grep -v "infwarerr" | grep -v "\(redefined the meaning of the math\|t cause unrecoverable errors\)" | grep -v "error-analysis")"]; then \
             echo "This latex error can be safely ignored"; \
         else \
             echo "****************************************"; \
             echo "There might be other latex errors:"; \
             echo "****************************************"; \
             echo "$$(grep -i "error" formatted.log | grep -v "errmessage" | grep -v "infwarerr" | grep -v "\(redefined the meaning of the math\|t cause unrecoverable errors\)" | grep -v "error-analysis")"; \
             echo "****************************************"; \
             echo "Check formatted.log for details!"; \
             exit 1; \
         fi
#	-$(LATEX) $*
	@echo '****************************************************************'
# vvvvvv For `latex` ONLY. Comment out for `pdflatex`
#	@dvips -j0 -t letter -o $(NAME).ps $(NAME).dvi
#	@ps2pdf -dPDFSETTINGS=/prepress $(NAME).ps $(NAME).pdf
# ^^^^^^^^^^^^^^^^^^^^^^^^
	@echo '******** Did you spell-check the paper? ********'

.PHONY: clean
clean:
	ls $(formattedS:=.*) | grep -v ".\(tex\|bib\|sty\)" | xargs rm -f
	rm -f *.bak *~
#	find -name "*.eps" | xargs rm -f


==> figures/combined_configuration_figure.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[scale=0.23]{images/combined_configurations.png}
\vspace{-5pt}
\caption{Overview of the three configurations used for the combined system which makes a prediction for whether \Comment{} is inconsistent ($P_{inconsistent}$) as well for the updated comment ($P_{comment}$). Modules are trained on either the full training set, including positive/inconsistent (+) and negative/consistent (-) examples, or only positive examples.}
\label{fig:combined_configs}
\end{figure*}

